PaCHash: Packed and Compressed Hash Tables

We introduce PaCHash, a hash table that stores its objects contiguously in an array without intervening space, even if the objects have variable size. In particular, each object can be compressed using standard compression techniques. A small search data structure allows locating the objects in constant expected time. PaCHash is most naturally described as a static external hash table where it needs a constant number of bits of internal memory per block of external memory. Here, in some sense, PaCHash beats a lower bound on the space consumption of k-perfect hashing. An implementation for fast SSDs needs about 5 bits of internal memory per block of external memory, requires only one disk access (of variable length) per search operation, and has small internal search overhead compared to the disk access cost. Our experiments show that it has lower space consumption than all previous approaches even when considering objects of identical size.

==> Makefile <==
paper_size ?= a4
pdf_quality ?= printer

all: paper

clean:
	rm -rf paper.pdf
	rm -rf *.log *.aux *.bbl *.blg .toc *.out *.toc
	rm -rf rev.tex

RERUN = '(There were undefined references|Rerun to get (cross-references|the bars) right)'
RERUNBIB = 'No file.*\.bbl|Citation.*undefined'
UNDEFINED = '((Reference|Citation).*undefined)|(Label.*multiply defined)'

pdflatex = pdflatex -interaction=batchmode paper.tex
pdflatex_safe = (pdflatex -interaction=batchmode paper.tex || true)
bibtex = bibtex paper

paper:: *.tex
	@echo "====> LaTeX first pass"
	$(pdflatex) || cat paper.log
	@if grep -E -q $(RERUNBIB) paper.log ; then echo "====> BibTex" && $(bibtex) && echo "====> LaTeX BibTeX pass" && $(pdflatex_safe) ; fi
	@if grep -E -q $(RERUN) paper.log ; then echo "====> LaTeX rerun" && $(pdflatex_safe); fi;
	@if grep -E -q $(RERUN) paper.log ; then echo "====> LaTeX rerun" && $(pdflatex_safe); fi;
	@echo "====> Undefined references and citations:"
	@grep -E -i $(UNDEFINED) paper.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" paper.log || echo "None."

